Heat, Health, and Habitats: Analyzing the Intersecting Risks of Climate and Demographic Shifts in Austrian Districts

The impact of hot weather on health outcomes of a population is mediated by a variety of factors, including its age profile and local green infrastructure. The combination of warming due to climate change and demographic aging suggests that heat-related health outcomes will deteriorate in the coming decades. Here, we measure the relationship between weekly all-cause mortality and heat days in Austrian districts using a panel dataset covering $2015-2022$. An additional day reaching $30$ degrees is associated with a $2.4\%$ increase in mortality per $1000$ inhabitants during summer. This association is roughly doubled in districts with a two standard deviation above average share of the population over $65$. Using forecasts of hot days (RCP) and demographics in $2050$, we observe that districts will have elderly populations and hot days $2-5$ standard deviations above the current mean in just $25$ years. This predicts a drastic increase in heat-related mortality. At the same time, district green scores, measured using $10\times 10$ meter resolution satellite images of residential areas, significantly moderate the relationship between heat and mortality. Thus, although local policies likely cannot reverse warming or demographic trends, they can take measures to mediate the health consequences of these growing risks, which are highly heterogeneous across regions, even in Austria.

==> Info.tex <==
 However, we strongly recommend that you write concisely and stick to the following guidelines:

- Articles should ideally be no more than 11 typeset pages
- The main text should be no more than 4,500 words (not including 
   Abstract, Methods, References and figure legends)
- The title should be no more than 20 words, should describe the main 
   message of the article using a single scientifically accurate sentence, and should not contain puns or idioms
- The abstract should be no more than 200 words
- No Abbreviation List

For the main body of the text, there are no specific requirements. You can organise it in a way that best suits your research. However, the following structure will be suitable in many cases:

- Introduction (without subheadings)
- Results (with subheadings)
- Discussion (without subheadings)
- Methods

You should then follow the main body of text with:

- References (limited to 60 references, though not strictly enforced)
    -- LaTeX formats citations and references automatically using the bibliography records in your .bib file, which you can edit via the project menu. Use the cite command for an inline citation, e.g.  \cite{Hao:gidmaps:2014}.
- Acknowledgements (optional)
- Author contributions
- Data availability statement (mandatory)
- Additional Information (including a Competing Interests Statement)
- Figure legends (these are limited to 350 words per figure)
- Tables (maximum size of one page)

Please note, footnotes should not be used. 

Further limitations: 
- Display items are limited to 8 (figures and/or tables). 
    However, to enable typesetting of papers, we advise making the number of display items commensurate with your overall word length. So, for Articles of 2,000 words or less, we suggest including no more than 4 figures/tables.

    

 
Your submission must also include:

- A cover letter
- Individual figure files and optional supplementary information files

For data citations of datasets uploaded to e.g. \emph{figshare}, please use the \verb|howpublished| option in the bib entry to specify the platform and the link, as in the \verb|Hao:gidmaps:2014| example in the sample bibliography file.

\section*{Acknowledgements (not compulsory)}

Acknowledgements should be brief, and should not include thanks to anonymous referees and editors, or effusive comments. Grant or contribution numbers may be acknowledged.

\section*{Author contributions statement}

Must include all authors, identified by initials, for example:
A.A. conceived the experiment(s),  A.A. and B.A. conducted the experiment(s), C.A. and D.A. analysed the results.  All authors reviewed the manuscript. 

\section*{Additional information}

To include, in this order: \textbf{Accession codes} (where applicable); \textbf{Competing interests} (mandatory statement). 

The corresponding author is responsible for submitting a \href{http://www.nature.com/srep/policies/index.html#competing}{competing interests statement} on behalf of all authors of the paper. This statement must be included in the submitted article file.


==> old_introduction.tex <==
[j:needs more tension like the youtube guy from Chicago says. what is unique? there are papers that show that heat kills, that urban heat islands are a problem, that old people are more vulnerable to heat, that green vegetation and other tricks bring relief (btw we should have these citations grouped). there are papers that show that the world is getting hotter and older. are there papers that show this for entire countries? for 'western european' countries? are we just combining all the lego bricks into a coherent story for one country?]\\
What is the problem? What is unique? What is the readers question we try to answer?
At the beginning of the Summer of 2023, temperature records for the hottest day in the world during the measurement period and many highest temperature records in different countries have already been broken. The global warming caused by climate change directly influences the number of heat waves \cite{huber_extreme_nodate}. Even if we reach the climate goal of $1.5$ degrees Celsius, which seems unlikely at the moment, we end up with a hotter environment and, consequently, more heat days in the summer period \cite{mukherji_synthesis_nodate}, which we are already experiencing. 

Many countries in relatively temperate climates are unprepared for high temperatures and require large-scale heat resilience adaptation. As global warming due to climate change directly increases the number of heat waves and heat days\cite{huber_extreme_nodate}, improving heat resilience becomes more crucial than ever. A lot of work focuses on the implications heat has on human health \cite{iungman_cooling_2023, weilnhammer_extreme_2021} and other aspects of human lives, like human mobility \cite{massaro_spatially-optimized_2023}.

However, little work has been done to quantify the heat resilience of cities or municipalities, like in \cite{buzasi_comparative_2022} characterizing the heat resilience of Budapest and \cite{zong_mapping_2023} analyzing China's heat resilience. In preparation for the increase in heat days, we need to quantify a municipality's heat resilience and determine if specific interventions affect its resilience level. [J: needs more WHY]

Currently, more than half of the earth's population lives in cities covering less than $3\%$ of the Earth’s land surface \cite{massaro_spatially-optimized_2023}. With the growing world population, this situation will probably get more extreme in the next few years. One of the most significant issues is that most cities are not constructed in one go but grow to maximize living space, not prioritizing green spaces. Due to this, the number of urban heat islands increases, posing a risk to the population's health ~\cite{iungman_cooling_2023}. 

The rising number of heat days especially challenges countries with milder temperatures, like Austria, as they face unfamiliar problems and new obstacles. Many of these countries are unprepared for high temperatures and require large-scale heat resilience adaptation. According to \cite{miranda_change_2023}, the demand for cooling days will experience dramatic relative increases in countries like Austria, approximately $24\%$. This directly results in higher energy consumption and more emissions caused by air conditioners. 

Heat directly impacts our lives; not only does it affect our environment, but it also impacts our health and well-being. The estimated number of heat-related deaths in Europe has risen in the last few years; a study estimated approximately 62 000 heat-related deaths in Europe between 30 May and 4 September 2022 \cite{ballester_heat-related_2023}. It is important to note that the number of heat-related deaths steeply increased with age, and especially women above 80 years were affected. Furthermore, several studies \cite{hajdu_post-conception_2021, cil_extreme_2022, Leung_pregnancy_2022} reported that prenatal health, as well as clinically unobserved pregnancy loss rate, are impacted by heat days.
Heat directly impacts our lives; not only does it affect our environment, but it also impacts our health and well-being. The estimated number of heat-related deaths in Europe has risen in the last few years; a study estimated approximately $62,000$ heat-related deaths in Europe between 30 May and 4 September 2022 \cite{ballester_heat-related_2023}. The health impacts of heat are various and range from increased mortality \cite{ballester_heat-related_2023} to adverse effects on prenatal health or an increased clinically unobserved pregnancy loss rate \cite{hajdu_post-conception_2021, Leung_pregnancy_2022,hajdu2023climate}. -- sentence on mechanisms of heat causing death --

Many studies report a positive association between extreme heat events and cardiovascular mortality \cite{weilnhammer_extreme_2021}. Especially a high ratio of elderly people with cardiovascular disease is a common weak point for heat resilience \cite{buzasi_comparative_2022}. In Austria, cardiovascular diseases rank as the leading cause of death. Since the probability of cardiovascular diseases increases with age \cite{HKE_AUT}, a high ratio of people aged above $65$ years is an additional risk factor for heat resilience. 

Therefore, we propose a heat score for municipalities to show municipalities their heat resilience considering different factors from various data sources. We also would like to provide a glimpse into the future using demographic forecasts and different scenarios for heat day development. 


[J: missing the point that while local politics/administration can't do much to solve climate change at the macro level, there is significant evidence that they do have specific policy levers to improve quality of life and health outcomes during: greenery and health spending. More generally: having a sound budget matters so that they can make these investments.]

